Implicit Feedback for Dense Passage Retrieval: A Counterfactual Approach

In this paper we study how to effectively exploit implicit feedback in Dense Retrievers (DRs). We consider the specific case in which click data from a historic click log is available as implicit feedback. We then exploit such historic implicit interactions to improve the effectiveness of a DR. A key challenge that we study is the effect that biases in the click signal, such as position bias, have on the DRs. To overcome the problems associated with the presence of such bias, we propose the Counterfactual Rocchio (CoRocchio) algorithm for exploiting implicit feedback in Dense Retrievers. We demonstrate both theoretically and empirically that dense query representations learnt with CoRocchio are unbiased with respect to position bias and lead to higher retrieval effectiveness. We make available the implementations of the proposed methods and the experimental framework, along with all results at https://github.com/ielab/Counterfactual-DR.

==> sections/backup-introduction.tex <==
\section{Introduction} \label{intro}

Dense Retrievers (DRs) are retrieval and ranking approaches where a transformer-based deep language model (e.g., BERT~\cite{bibid}) is used to encode queries and documents in low dimensional embeddings (dense vectors), which are then used as representation for matching via vector similarity search. 
Although generally less effective than cross-encoder approaches such as mono-BERT~\cite{}, DRs offer much lower query latency, overcoming the main barrier to adoption of cross-encoder methods (high query latency and high computational cost).


Pseudo Relevance Feedback (PRF) assumes the top-ranked passages from any phase of retrieval contain relevant signals, and thus modifies the query by exploiting these signals. This is done with the intent of reducing the effect of query-passage vocabulary mismatch and improve search effectiveness. PRF methods have recently been adapted and developed for DRs, further boosting DRs' search effectiveness, closing the gap with the more effective cross-encoder approaches.

In this paper, we are interested to investigate the use of feedback mechanisms to improve search effectiveness beyond the PRF setting, i.e. that of assuming the top-k documents are relevant. In particular, in this paper we investigate the application of a method originally proposed for PRF with dense retrievers in the different context of implicit relevance signal. Implicit relevance signals consist of users interactions with the search engine result page (SERP) that may be indicative of the relevance of the items in the SERP: this may be clicks~\cite{agichtein2006improving,joachims2017accurately}, reading time~\cite{kelly2001reading},  but can further extend to physiological, psychological and other behavioural signals~\cite{arapakis2009using,moshfeghi2013effective}. In this paper, we restrict our consideration of implicit relevance signals to click-through data, following the long-standing practice in online learning to rank and counterfactual learning to rank~\cite{bibid}. 

The key idea we put forward in this paper is to adapt current PRF methods for DRs to deal with implicit relevance feedback in terms of clicks. A first sight, this can be achieved by simply removing the PRF assumption that the top-k search results are relevant and therefore form the relevance signal. This assumption can be replaced by the assumption that the clicked search results are what constitutes the relevance signals, and thus are the input to the implicit relevance feedback (IRF) mechanism. This intuition is depicted in Figure~\ref{fig:implicit} where the dense representation of the query $\vec{q}$ is aggregated according to the IRF mechanism with the dense representation of the clicked documents $\vec{d_1}$ and $\vec{d_3}$, to create the updated query $\vec{q}'$. 

\begin{figure}[t]
	\includegraphics[width=0.9\linewidth]{implicit.png}
	\vspace{-10pt}
	\caption{Implicit relevance feedback for DR.\vspace{-20pt}}
	\label{fig:implicit}
\end{figure}

The adaptation of current PRF methods for DRs to implicit relevance feedback signals such as click-through data , however, presents three key challenges.
%\begin{itemize}
%	\item 
	
	\textbf{Challenge 1 (click bias):} it is well known that the click signal presents a number of biases~\cite{bibid}, such as position bias. Then, what is the impact of this bias on the effectiveness of relevance feedback methods for DRs when clicks are used as relevance signal? How can this bias be removed from the click signal -- and does this improve search effectiveness?
	
	To investigate and address this challenge, we firs study the impact of implicit relevance feedback on the effectiveness of DRs under different user conditions and click bias. We then propose a counterfactual IRF method for DRs, based on advances in counterfactual and online learning to rank~\cite{bibid}, that mitigates the impact of bias in the click signal when used for implicit feedback. Specifically, our method relies on a historic click log to estimate the likelihood of position bias associated to a query $\vec{q}$. This is then used to adjust the weight of the dense representation associated to a feedback document $\vec{d}$ when aggregating this signal with that from other documents and the original query $\vec{q}$ to compute the new dense query representation $\vec{q}'$. 
	
	%\item 
	\textbf{Challenge 2 (datasets):} the training of DRs requires large datasets, such as MS MARCO, that contain both textual passages and relevance labels. These datasets however do not have corresponding click data to be used as implicit feedback to support our investigation. Then, how can existing large datasets for training and evaluating DRs be extended with click information? 
	
	To address this challenge, we use the evaluation practice developed in online learning to rank, where click models are used to simulate user interactions. This allows us to simulate clicks on passage ranking collections used to study DRs.
	
	\textbf{Challenge 3 (counterfactual IRF with unseen queries):} our counterfactual IRF method requires that, for any given query to be scored, the historic click log contains interactions with SERPs for that query. While this is a reasonable expectation for popular queries, it is reasonable to expect that users will enter queries that are not present in the historic click log and thus it is desirable for the IRF method to be used in such a context. What strategy can then be used to adapt the proposed counterfactual IRF method to cases in which the query has not been previously observed in the historic click log?
	
	To address this final challenge, we first identify a strategy to generate new queries not in but yet related to\footnote{Such that the signals from the historic click log bear a valuable signal for the unseen queries.} the historic query log we create as dataset for our counterfactual IRF. We then devise a simple but effective strategy to identify the signal from the historic click log to be used to de-bias the click signal from the current query for our counterfactual IRF method.
	
%\end{itemize}

In summary, this paper explores a novel research direction: that of applying relevance feedback mechanisms for DRs, currently limited to PRF settings, to implicit relevance feedback settings, such as the implicit signal obtained from click-through data. With this respect, we also demonstrate how evaluation practices developed for online learning to rank can be adopted to this context. In addition, we show that the click signal can be highly informative, making these methods highly effective. On the other hand, we show that the noise and bias typically found in click-through data (and likely present in other types of implicit feedback)  have a significant detrimental effect on IRF methods for DRs. To address this issue we contribute a novel counterfactual IRF method for DRs, called Counterfactual Rocchio (CoRocchio) and investigate the key factors that influence its effectiveness. 



